Understanding Counting Mechanisms in Large Language and Vision-Language Models

Counting is one of the fundamental abilities of large language models (LLMs) and large vision-language models (LVLMs). This paper examines how these foundation models represent and compute numerical information in counting tasks. We use controlled experiments with repeated textual and visual items and analyze counting in LLMs and LVLMs through a set of behavioral, observational, and causal mediation analyses. To this end, we design a specialized tool, CountScope, for the mechanistic interpretability of numerical content. Results show that individual tokens or visual features encode latent positional count information that can be extracted and transferred across contexts. Layerwise analyses reveal a progressive emergence of numerical representations, with lower layers encoding small counts and higher layers representing larger ones. We identify an internal counter mechanism that updates with each item, stored mainly in the final token or region. In LVLMs, numerical information also appears in visual embeddings, shifting between background and foreground regions depending on spatial composition. We further reveal that models rely on structural cues such as separators in text, which act as shortcuts for tracking item counts and strongly influence the accuracy of numerical predictions. Overall, counting emerges as a structured, layerwise process in LLMs and follows the same general pattern in LVLMs, shaped by the properties of the vision encoder.

==> sec/91_related_work.tex <==
\section{Related Work}
\label{sec:related work}

\paragraph{Counting competence and evaluation instability in LLMs.}
A growing body of evidence suggests that current LLMs exhibit \emph{fragile} counting ability even on simple tasks.
Fu et al.\ report systematic failures on character-counting queries (e.g., counting occurrences of a letter), showing that errors persist across models and stem from the intrinsic difficulty of repetition-tracking rather than token frequency or exposure~\cite{fu2024letters}.
Zhang et al.\ argue from computational and empirical perspectives that transformer LLMs lack an inherent mechanism for unbounded counting and that common subword tokenization schemes can further degrade performance by obscuring item boundaries~\cite{zhang2024tokenization}.
Complementing these findings, Ball et al.\ show that performance on deterministic tasks such as counting is highly sensitive to seemingly benign prompt/content variations, cautioning against extrapolating from single-prompt evaluations (the \emph{fixed-effect fallacy})~\cite{canwecount2024}.
Orthogonally, Yehudai et al.\ analyze \emph{when} transformers can count and show that exact counting of a token’s frequency in a string is feasible when the model state dimension scales linearly with context length, providing conditions and constructions that clarify capability limits~\cite{yehudai2024whencount}.
Together, these works motivate analyses that go beyond aggregate accuracy to \emph{how} numerical information is internally represented and why surface behavior can flip under minor rephrasings.

\vspace{-3mm}
\paragraph{Mechanistic and causal analyses of numeracy.}
A parallel line of work uses controlled tasks and interpretability tools to probe internal number mechanisms.
Golkar et al.\ introduce a contextual counting task and show that autoregressive transformers can learn effective counting strategies; intriguingly, removing positional embeddings or using rotary encodings changes where and how the mechanism emerges~\cite{golkar2024contextual}.
{Stolfo et al.\ apply a causal mediation analysis framework to arithmetic reasoning, intervening on layerwise activations to identify mid--late layers and specific components that causally mediate correct versus incorrect arithmetic predictions~\cite{stolfo2023cma}. In our work, we adopt compatible mediation-style \emph{effect scores} to quantify causal influence of activations on numeric outputs, in spirit similar to their CMA-based scoring.}
Shah et al.\ probe numeral embeddings and hidden states, finding cognitive-like magnitude effects (distance, ratio, size), hinting at an emergent ``mental number line''~\cite{shah2023numeric}.
Our work builds on these insights but focuses specifically on \emph{counting} and contributes a unified causal picture across both text-only LLMs and LVLMs: we show that latent count states are (i) primarily stored in contextual activations, (ii) concentrate in the final token/region, (iii) emerge progressively across layers, and (iv) are \emph{linearly additive} and transferable across contexts.

\vspace{-3mm}
\paragraph{Counting in LVLMs and the role of vision.}
In multimodal models, counting introduces additional challenges due to visual encoding, spatial aggregation, and modality fusion.
Paiss et al.\ demonstrate that CLIP---despite strong retrieval---often ignores cardinality; they improve counting via a counting-aware contrastive loss and show broader attentional coverage after fine-tuning~\cite{paiss2023clipcount}.
Guo et al.\ expose striking failures in \emph{compositional} counting (multiple object types), indicating unreliable binding between category and quantity~\cite{guo2025vlmcount}.
\emph{LLaVA-Interp} analyzes LLaVA’s \emph{visual} tokens with Logit Lens and ablations, showing that visual representations increasingly align with vocabulary space across layers and can project onto content-descriptive tokens (including numerals), suggesting image-derived numeric cues may surface in LM-space and relate to counting behavior~\cite{neo2024llavainterp}.
Consistent with these observations, we find that LVLMs’ count evidence often resides in both foreground and \emph{background} visual tokens and is more sensitive to layout, density, and resolution than in text-only models.
Our causal patching further shows that, unlike text, the most informative visual region is not always tied to the last object, reflecting pre-decoder global integration in the vision stack.

\vspace{-3mm}
\paragraph{Causal intervention toolkit and patch-based probes.}
Methodologically, our study connects to activation-level interpretability: activation/mean/interchange patching, key--value (attention) interventions, and mediation analysis; and to layerwise readout probes such as the original \emph{Logit Lens} and its learned variant \emph{Tuned Lens}~\cite{nostalgebraist2020logitlens,belrose2023tunedlens}.
\emph{Patchscopes} unifies patching/inspection configurations and leverages stronger models to explain internal representations in natural language, enabling expressive cross-layer analyses~\cite{ghandeharioun2024patchscopes}.
We introduce \textbf{CountScope}, a lightweight target-context probe tailored to numerical decoding, enabling precise, layerwise and token/patch-level localization of latent count states in both LLMs and LVLMs.
Beyond corroborating prior observations (e.g., layerwise emergence, shortcutting on separators), our causal experiments uncover (a) \emph{internal latent counters} that update across items and transfer across contexts, (b) \emph{type-specific counters} that can \emph{reset} in polytypic lists, and (c) a \emph{max-latent-count} effect whereby the model’s final prediction often reflects the maximum latent count present in context rather than a simple sum.


==> tables/LLM_NoSeperator.tex <==
\begin{table}[t]
\centering

\resizebox{\linewidth}{!}{
\begin{tabular}{@{}llcccc@{}}
\toprule
\textbf{Model} & \textbf{Category} &
\multicolumn{2}{c}{\textbf{List-first}} & \multicolumn{2}{c}{\textbf{Question-first}} \\
\cmidrule(lr){3-4}\cmidrule(lr){5-6}
 &  & Specific & General &                              Specific & General \\
\midrule
\multirow{3}{*}{\textbf{Qwen2.5}}
  & Monotypic          & 97.22 & 97.22 & 100.00 & 100.00 \\
  & Polytypic—Replicate    & 84.84 & 27.43 & 77.94 & 31.61 \\
  & Polytypic—Unique      & 62.60 & 75.38 & 99.76 & 76.15 \\
\cmidrule(l){2-6}
\multirow{3}{*}{\textbf{Llama3}}
  & Monotypic          & 19.44 & 19.44 & 25.00 & 25.00 \\
  & Polytypic—Replicate    & 79.27 & 0.63 & 83.33 & 00.00 \\
  & Polytypic—Unique      & 100.00 & 30.77 & 100.00 & 6.15 \\
\bottomrule
\end{tabular}
}
\caption{no separator.}
\label{tab:llm_noseparator}
\end{table}

==> tables/LLM_behavioral_10To19.tex <==
\begin{table}[t] % or [htbp]
\centering
\caption{LLM behavioral 10--19 objects}
\label{tab:llm_behavioral_10_19}

\begingroup
\setlength{\tabcolsep}{1pt} % tighter columns

\resizebox{\linewidth}{!}{
\begin{tabular}{@{}llcccc@{}}
\toprule
\textbf{Model} & \textbf{Category} &
\multicolumn{2}{c}{\textbf{List-first}} &
\multicolumn{2}{c}{\textbf{Question-first}} \\
\cmidrule(lr){3-4}\cmidrule(lr){5-6}
 &  & Specific & General & Specific & General \\
\midrule
\multirow{3}{*}{\textbf{Qwen2.5}}
  & Monotypic          & 91.67 & 91.67 & 91.67 & 91.67 \\
  & Polytypic-Repeated & 88.13 & 91.96 & 88.34 & 70.90 \\
  & Polytypic-Unique   & 57.71 & 100.00 & 89.13 & 100.00 \\
\cmidrule(l){2-6}
\multirow{3}{*}{\textbf{Qwen2.5-VL}}
  & Monotypic          & 100.00 & 100.00 & 100.00 & 100.00 \\
  & Polytypic-Repeated & 92.39  & 40.21  & 80.24  & 48.81 \\
  & Polytypic-Unique   & 100.00 & 100.00 & 100.00 & 100.00 \\
\midrule
\multirow{3}{*}{\textbf{Llama3}}
  & Monotypic          & 94.44 & 94.44 & 94.44 & 94.44 \\
  & Polytypic-Repeated & 94.35 & 6.23   & 89.85 & 1.41  \\
  & Polytypic-Unique   & 100.00 & 99.23 & 78.38 & 100.00 \\
\cmidrule(l){2-6}
\multirow{3}{*}{\textbf{InternVL3.5}}
  & Monotypic          & 100.00 & 100.00 & 100.00 & 100.00 \\
  & Polytypic-Repeated & 99.36  & 56.05  & 99.77  & 64.58 \\
  & Polytypic-Unique   & 100.00 & 98.46  & 100.00 & 100.00 \\
\bottomrule
\end{tabular}
}

\endgroup
\end{table}


==> tables/LLM_seperator_old.tex <==

\begin{table}[t]
\centering
\resizebox{\linewidth}{!}{
\begin{tabular}{@{}lllcccccc@{}}
\toprule
\textbf{Model} & \textbf{Question type} & \textbf{Category} &
\multicolumn{3}{c}{\textbf{List-first}} &
\multicolumn{3}{c}{\textbf{Question-first}} \\
\cmidrule(lr){4-6}\cmidrule(lr){7-9}
 &  &  & Replace & Delete & Extra & Replace & Delete & Extra \\
\midrule

\multirow{6}{*}{\textbf{Qwen2.5}} &
  \multirow{3}{*}{General} &
  Monotypic               & 8.33 & 55.56 & 8.33 & 8.33 & 13.89 & 16.67 \\
 & & Polytypic--Replicate  & 5.53 & 8.29 & 11.95 &  6.32 & 8.04 & 16.75 \\
 & & Polytypic--Unique    & 17.69 & 22.30 & 76.57 & 32.30 & 27.69 & 61.21 \\
\cmidrule(l){2-9}
 & \multirow{3}{*}{Specific} &
  Monotypic               & 8.33 & 55.56 & 8.33 & 8.33 & 11.56 & 16.67 \\
 & & Polytypic--Replicate  & 73.22 & 71.21 & 23.85 & 60.79 & 58.15 & 39.23 \\
 & & Polytypic--Unique    & 66.19 & 55.32 & 73.12 & 88.53 & 92.11 & 85.66 \\
\midrule

\multirow{6}{*}{\textbf{Llama3}} &
  \multirow{3}{*}{General} &
  Monotypic               & 16.67 & 8.33 & 55.56 & 11.11 & 11.11 & 44.44 \\
 & & Polytypic--Replicate  & 1.95 & 0.66 & 11.02 & 0.41 & 0.14 & 0.84 \\
 & & Polytypic--Unique    & 40.00 & 14.62 & 76.15 & 43.08 & 3.85 & 93.85 \\
\cmidrule(l){2-9}
 & \multirow{3}{*}{Specific} &
  Monotypic               & 16.67 & 8.33 & 55.56 & 16.67 & 11.11 & 44.44 \\
 & & Polytypic--Replicate  & 69.02 & 64.55 & 84.57 & 73.10 & 7.025 & 77.53 \\
 & & Polytypic--Unique    & 89.09 & 99.04 & 100.00 & 83.27 & 90.80 & 79.09 \\
\bottomrule
\end{tabular}
}
\caption{separator.}
\label{tab:llm_separator}
\end{table}

==> tables/LVLM_size_sparsity_qwen.tex <==
\begin{table}[t]
\centering
\setlength{\tabcolsep}{1pt}
\label{tab:res_size_density_3}
\begin{tabular}{@{}cccccccc@{}}
\toprule
\multirow{2}{*}{\textbf{Resolution}} &
\multicolumn{2}{c}{\textbf{Size 14}} &
\multicolumn{2}{c}{\textbf{Size 28}} &
\multicolumn{2}{c}{\textbf{Size 56}} \\
\cmidrule(lr){2-3}\cmidrule(lr){4-5}\cmidrule(lr){6-7}
 & Sparse & Dense
 & Sparse & Dense
 & Sparse & Dense \\
\midrule
280$\times$280
 & 55.43 & 46.09
 & 70.28 & 74.52
 & 75.92 & 69.08 \\
560$\times$560
 & 33.24 & 30.94
 & 66.10 & 63.87
 & 69.55 & 66.95 \\
\bottomrule
\end{tabular}

\caption{VLM, Accuracy by resolution, object size, and density mode.Qwen2.5}
\end{table}

==> tables/VLM_RowColumn.tex <==
\begin{table}[t] % or [htbp]
\centering
\caption{Column/Row performance of InternVL3.5 and Qwen2.5-VL}
\setlength{\tabcolsep}{1pt}
\label{tab:panel_mixed}
\resizebox{\linewidth}{!}{
\begin{tabular}{@{}lllcccc@{}}
\toprule
\textbf{Model} & \textbf{Layout} & \textbf{Category} &
\multicolumn{2}{c}{\textbf{List-first}} &
\multicolumn{2}{c}{\textbf{Question-first}} \\
\cmidrule(lr){4-5}\cmidrule(lr){6-7}
 &  &  & Specific & General & Specific & General \\
\midrule
\multirow{6}{*}{\textbf{InternVL3.5}}
  & \multirow{3}{*}{Row}
    & Monotypic          & 69.44 & 72.22 & 66.67 & 77.78 \\
  & & Polytypic-Repeated & 83.84 & 68.40 & 69.62 & 72.65 \\
  & & Polytypic-Unique   & 83.39 & 89.23 & 81.72 & 94.62 \\
\cmidrule(lr){2-7}
  & \multirow{3}{*}{Column}
    & Monotypic          & 72.22 & 72.22 & 83.33 & 77.78 \\
  & & Polytypic-Repeated & 84.41 & 77.51 & 70.75 & 71.20 \\
  & & Polytypic-Unique   & 83.15 & 83.85 & 82.44 & 84.62 \\
\midrule
\multirow{6}{*}{\textbf{Qwen2.5-VL}}
  & \multirow{3}{*}{Row}
    & Monotypic          & 50.00 & 61.11 & 50.00 & 61.11 \\
  & & Polytypic-Repeated & 79.06 & 57.99 & 77.57 & 61.97 \\
  & & Polytypic-Unique   & 77.66 & 80.77 & 88.29 & 79.23 \\
\cmidrule(lr){2-7}
  & \multirow{3}{*}{Column}
    & Monotypic          & 25.00 & 41.67 & 41.67 & 47.22 \\
  & & Polytypic-Repeated & 78.49 & 42.97 & 72.86 & 48.36 \\
  & & Polytypic-Unique   & 79.57 & 80.77 & 89.37 & 84.62 \\
\bottomrule
\end{tabular}
}
\end{table}


==> tables/VLM_RowColumn_qwen.tex <==
\begin{table}[t] % or [htbp]
\centering
\caption{Column Row Qwen2.5-VL}
\setlength{\tabcolsep}{1pt}
\label{tab:panel_qwen}
\begin{tabular}{@{}llcccc@{}}
\toprule
\textbf{Layout} & \textbf{Category} &
\multicolumn{2}{c}{\textbf{List-first}} &
\multicolumn{2}{c}{\textbf{Question-first}} \\
\cmidrule(lr){3-4}\cmidrule(lr){5-6}
 &  & Specific & General & Specific & General \\
\midrule
\multirow{3}{*}{\textbf{Row}}
  & Monotypic          & 50.00 & 61.11 & 50.00 & 61.11 \\
  & Polytypic-Repeated & 79.06 & 57.99 & 77.57 & 61.97 \\
  & Polytypic-Unique   & 77.66 & 80.77 & 88.29 & 79.23 \\
\cmidrule(l){2-6}
\multirow{3}{*}{\textbf{Column}}
  & Monotypic          & 25.00 & 41.67 & 41.67 & 47.22 \\
  & Polytypic-Repeated & 78.49 & 42.97 & 72.86 & 48.36 \\
  & Polytypic-Unique   & 79.57 & 80.77 & 89.37 & 84.62 \\
\bottomrule
\end{tabular}
\end{table}


==> tables/offline_question_patching.tex <==
\begin{table}[t]
\centering
\caption{Mean drop in the probability of the ground-truth count when applying offline zero patching to context (list) tokens versus question tokens, as a function of list length (LLM). Higher values indicate that masking removes more count-relevant information from that part of the prompt.}
\label{tab:offline_zero_context_vs_question}

\begingroup
\setlength{\tabcolsep}{6pt}

\begin{tabular}{@{}ccc@{}}
\toprule
\textbf{Count} &
\textbf{Mean drop (context masked)} &
\textbf{Mean drop (question masked)} \\
\midrule
1 & 0.0000 & 0.0000 \\
2 & 0.0654 & 0.0002 \\
3 & 0.6832 & 0.0000 \\
4 & 0.9806 & 0.0000 \\
5 & 0.5606 & 0.0000 \\
6 & 0.8135 & 0.0000 \\
7 & 0.7917 & 0.0000 \\
8 & 0.9497 & 0.2563 \\
9 & 0.9862 & 0.0008 \\
\bottomrule
\end{tabular}

\endgroup
\end{table}


==> tables/offline_question_patching_vlm.tex <==
\begin{table}[t]
\centering
\caption{Mean drop in the probability of the ground-truth count when applying offline zero patching to prompt tokens versus image patches in an LVLM, as a function of object count. Higher values indicate that masking removes more count-relevant information from that modality.}
\label{tab:offline_zero_context_vs_question}

\begingroup
\setlength{\tabcolsep}{6pt}

\begin{tabular}{@{}ccc@{}}
\toprule
\textbf{Count} &
\textbf{Mean drop (image patch masked)} &
\textbf{Mean drop (prompt token masked)} \\
\midrule
1 & 0.9539 & 0.0187 \\
2 & 0.9691 & 0.0167 \\
3 & 0.9535 & 0.0304 \\
4 & 0.8789 & 0.0617 \\
5 & 0.7605 & 0.0714 \\
6 & 0.6363 & 0.1119 \\
7 & 0.5181 & 0.0617 \\
8 & 0.4916 & 0.0812 \\
9 & 0.4515 & 0.0330 \\
\bottomrule
\end{tabular}

\endgroup
\end{table}

